PersuasiveToM: A Benchmark for Evaluating Machine Theory of Mind in Persuasive Dialogues

The ability to understand and predict the mental states of oneself and others, known as the Theory of Mind (ToM), is crucial for effective social scenarios. Although recent studies have evaluated ToM in Large Language Models (LLMs), existing benchmarks focus on simplified settings (e.g., Sally-Anne-style tasks) and overlook the complexity of real-world social interactions. To mitigate this gap, we propose PersuasiveToM, a benchmark designed to evaluate the ToM abilities of LLMs in persuasive dialogues. Our framework contains two core tasks: ToM Reasoning, which tests tracking of evolving desires, beliefs, and intentions; and ToM Application, which assesses the use of inferred mental states to predict and evaluate persuasion strategies. Experiments across eight leading LLMs reveal that while models excel on multiple questions, they struggle with the tasks that need tracking the dynamics and shifts of mental states and understanding the mental states in the whole dialogue comprehensively. Our aim with PersuasiveToM is to allow an effective evaluation of the ToM reasoning ability of LLMs with more focus on complex psychological activities. Our code is available at https://github.com/Yu-Fangxu/PersuasiveToM.

==> fig_texts/desire_er.tex <==
\begin{figure*}[t]
  \centering %
\begin{mybox}[Prompt for 1D-ARC]
\begin{obeylines}
You are provided with a series of input-output pairs, where each value from 'a' to 'j' represents a different color, and '.' denotes a blank cell. For example, [['.','a','.'],['.','.','b']] represents a grid with 2 rows and 3 columns, where color 'a' is at position (1,0) and color 'b' is at position (2,1). 

Coordinates are expressed in 2D positions (row, col), with 'row' indicating the row number and 'col' indicating the column number, both using zero-based indexing. The input-output pairs may not cover all possibilities, so you should infer the simplest possible relationship between them.

Your task is to reason through a sequence of Python functions that can transform the input grid into the output grid. Please strictly follow this process to form the appropriate Python function.

[STATEMENT]
You have the following input-output pairs:
[Initial Grid State]:
<init\_state>

Based on the provided list of Python functions, select the appropriate function to achieve the transformation from the input to the output:

<python\_function>

Now, please choose one function from the above list:
<action>
\end{obeylines}
\end{mybox}
\vspace{-12pt}
\caption{Prompt template for abstraction reasoning task.}
\label{fig:prompt-template-arc}
\end{figure*}


